FoodPuzzle: Developing Large Language Model Agents as Flavor Scientists

Flavor development in the food industry is increasingly challenged by the need for rapid innovation and precise flavor profile creation. Traditional flavor research methods typically rely on iterative, subjective testing, which lacks the efficiency and scalability required for modern demands. This paper presents three contributions to address the challenges. Firstly, we define a new problem domain for scientific agents in flavor science, conceptualized as the generation of hypotheses for flavor profile sourcing and understanding. To facilitate research in this area, we introduce the FoodPuzzle, a challenging benchmark consisting of 978 food items and 1,766 flavor molecules profiles. We propose a novel Scientific Agent approach, integrating in-context learning and retrieval augmented techniques to generate grounded hypotheses in the domain of food science. Experimental results indicate that our model significantly surpasses traditional methods in flavor profile prediction tasks, demonstrating its potential to transform flavor development practices.

==> figs/task_2_results.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{lcc}
\toprule
\small
\textbf{Category} & \textbf{Model} & \textbf{Accuracy (\%)} \\
\midrule
\multirow{3}{*}{Foundation LLMs} & LLaMA3-8B-instruct & - \\
                                 & Gemini1.5 Pro & 19 \\
                                 & GPT-3.5 Turbo & 18 \\
\midrule
\multirow{3}{*}{RAG-enhanced} & LLaMA3-8B-instruct & - \\
 & Gemini1.5 Pro & 23 \\
 & GPT-3.5 & 21 \\
\midrule
\multirow{2}{*}{Domain-Specific LLMs} & MolT5 \cite{edwards2022translation} & 0 \\
                                      & Bio-T5 \cite{pei-etal-2023-biot5} & 0 \\

\bottomrule
\end{tabular}
\caption{Model IoU scores for Molecule Profile Completion}
\label{tab:iou}
\end{table*}

==> sections/introduction_benchmark.tex <==
\section{  Introduction}

\muhao{Need to specify the scope of the studied problem. autonomous agent is too broad. Looks like this work is for hypothesis generation.}

%\muhao{Generally would avoid ``AI agents'' that is too broad. Could use LLM agents instead.}
The burgeoning demand for novel and appealing flavors in the food industry necessitates expedited innovation cycles without compromising on quality \muhao{+citation}. 
Traditional methods reliant on manual assessment and human expertise are inherently limited by time constraints and subjectivity, thus hindering the pace of flavor development \muhao{+citation}. 
In addition, the complexity of flavor interactions and the vast array of available ingredients present formidable challenges for food scientists in optimizing flavor profiles \muhao{+citation}. 
\tenghao{Would really appreciate some food science insights/citations in this first paragrpah @Emily}

Recent advancements in Large Language Models (LLMs) have revolutionized traditional scientific methodologies across a broad spectrum of disciplines. In fields ranging from biology and chemistry to physics and materials science, researchers have employed LLM technologies to analyze complex datasets, uncover hidden patterns, and significantly accelerate the pace of scientific discovery \cite{horawalavithana-etal-2022-foundation,Singhal2022LargeLM, o2023bioplanner, Hong2024DataIA, song-etal-2023-matsci}. This trend highlights the transformative potential of LLMs in reshaping traditional paradigms and catalyzing breakthroughs, particularly in food science research. Traditionally, the process of ingredient sourcing and evaluation for flavor development has been labor-intensive and subjective, relying on time-consuming iterations. \tenghao{maybe cite some food science papers @Emily }This paper explores how the integration of LLMs can streamline and enhance these processes, using cutting-edge technologies to optimize crucial aspects of flavor development. However, the application of LLMs in food science is hindered by a significant barrier: the absence of high-quality, domain-specific datasets. Most LLMs are trained on generic data from the web, which often lacks the detailed, specialized knowledge required for accurate flavor prediction.
% We aim to leverage the broad capabilities of LLM agents as documented in the recent literature, setting the stage for significant advancements in food science.

To address these challenges, this paper introduces ``FoodPuzzle'' a novel benchmark designed to assess and improve the performance of autonomous scientists within the food science domain. To gather data for our study on flavor, molecule prediction and analysis, we turn to the Flavor DB \cite{garg2018flavordb}. FlavorDB is a comprehensive database dedicated to flavor molecules, designed to facilitate a deeper understanding of the chemistry behind taste and smell. The database includes detailed information on 25,595 flavor molecules, of which 2,254 are specifically noted for their presence in 936 natural ingredients, providing a rich resource for both academic and industry research into flavor profiles.


Our primary contribution through this paper is the creation of the FoodPuzzle dataset, which aims to fill the existing void of high-quality, domain-specific training data. This dataset is structured to mirror real-world challenges in flavor development, thus enabling deeper insights into flavor compound interactions and training models to predict and recommend innovative flavor combinations effectively.

Despite the promising potential of LLMs in aiding flavor development, several challenges must be addressed to realize its full benefits. LLMs that are pretrained on Web corpora may lack domain-specific knowledge, leading to limitations in accurately seeking for evidence, understanding and interpreting complex flavor interactions \cite{yao2023knowledge, wu2024pmc}. This can result in ``hallucinations'' where the models generate inaccurate predictions or suggest implausible ingredient combinations. Especially in the domain of food science, where the relevant knowledge is lacking on the internet and language models are not optimized for this specialized domain, addressing this challenge is essential for ensuring the reliability and relevance of LLMs for food science. Although there are efforts to infuse world knowledge into LLMs to aid reasoning within specific scientific domains \cite{munikoti2023evaluating}, LLMs frequently encounter difficulties in effectively seeking and evaluating evidence. This deficiency undermines their ability to leverage relevant, high-quality information during the reasoning process, thereby compromising the accuracy of their outputs in a specialized field. %such as flavor development in food science.

Given the complexity of the FoodPuzzle task and the current limitations of available data, our second major contribution is the development of a specialized autonomous scientist method. This approach uses a Retrieval-Augmented Generation (RAG) framework specifically tailored for hypothesis generation in food science. By ensuring that suggestions are grounded in scientific evidence, this method not only improves the accuracy and reliability of the model’s outputs but also provides traceable justifications for its predictions.

By introducing FoodPuzzle, this paper sets a crucial benchmark for the application of advanced AI technologies in flavor science. It addresses the critical need for high-quality datasets and enhances the transparency and explainability of the predictive processes, paving the way for broader acceptance and practical use of LLMs in the food industry.

==> sections/methodology.tex <==

\subsection{Results}

\section{Future Directions}
